Conversational AI Threads for Visualizing Multidimensional Datasets

Generative Large Language Models (LLMs) show potential in data analysis, yet their full capabilities remain uncharted. Our work explores the capabilities of LLMs for creating and refining visualizations via conversational interfaces. We used an LLM to conduct a re-analysis of a prior Wizard-of-Oz study examining the use of chatbots for conducting visual analysis. We surfaced the strengths and weaknesses of LLM-driven analytic chatbots, finding that they fell short in supporting progressive visualization refinements. From these findings, we developed AI Threads, a multi-threaded analytic chatbot that enables analysts to proactively manage conversational context and improve the efficacy of its outputs. We evaluate its usability through a crowdsourced study (n=40) and in-depth interviews with expert analysts (n=10). We further demonstrate the capabilities of AI Threads on a dataset outside the LLM's training corpus. Our findings show the potential of LLMs while also surfacing challenges and fruitful avenues for future research.

==> Makefile <==
#
# Makefile for acmart package
#
# This file is in public domain
#
# $Id: Makefile,v 1.10 2016/04/14 21:55:57 boris Exp $
#

PACKAGE=acmart


PDF = $(PACKAGE).pdf acmguide.pdf

BIBLATEXFILES= $(wildcard *.bbx) $(wildcard *.cbx) $(wildcard *.dbx) $(wildcard *.lbx)
SAMPLEBIBLATEXFILES=$(patsubst %,samples/%,$(BIBLATEXFILES))

all:  ${PDF} ALLSAMPLES

%.pdf:  %.dtx   $(PACKAGE).cls
	pdflatex $<
	- bibtex $*
	pdflatex $<
	- makeindex -s gind.ist -o $*.ind $*.idx
	- makeindex -s gglo.ist -o $*.gls $*.glo
	pdflatex $<
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $*.log) \
	do pdflatex $<; done


acmguide.pdf: $(PACKAGE).dtx $(PACKAGE).cls
	pdflatex -jobname acmguide $(PACKAGE).dtx
	- bibtex acmguide
	pdflatex -jobname acmguide $(PACKAGE).dtx
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' acmguide.log) \
	do pdflatex -jobname acmguide $(PACKAGE).dtx; done

%.cls:   %.ins %.dtx
	pdflatex $<


ALLSAMPLES: $(SAMPLEBIBLATEXFILES)
	cd samples; pdflatex samples.ins; cd ..
	for texfile in samples/*.tex; do \
		pdffile=$${texfile%.tex}.pdf; \
		${MAKE} $$pdffile; \
	done

samples/%: %
	cp $^ samples


samples/$(PACKAGE).cls: $(PACKAGE).cls
samples/ACM-Reference-Format.bst: ACM-Reference-Format.bst

samples/abbrev.bib: ACM-Reference-Format.bst
	perl -pe 's/MACRO ({[^}]*}) *\n/MACRO \1/' ACM-Reference-Format.bst \
	| grep MACRO | sed 's/MACRO {/@STRING{/' \
	| sed 's/}  *{/ = /' > samples/abbrev.bib 


samples/%.bbx: %.bbx
samples/%.cbx: %.cbx
samples/%.dbx: %.dbx
samples/%.lbx: %.lbx

samples/%.pdf:  samples/%.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex-dev $(notdir $<); done

samples/sample-sigconf-biblatex.pdf: samples/sample-sigconf-biblatex.tex $(SAMPLEBIBLATEXFILES)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	- cd $(dir $@) && biber $(notdir $(basename $<))
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex-dev $(notdir $<); done

samples/sample-acmsmall-biblatex.pdf: samples/sample-acmsmall-biblatex.tex $(SAMPLEBIBLATEXFILES)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	- cd $(dir $@) && biber $(notdir $(basename $<))
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex-dev $(notdir $<); done

samples/sample-xelatex.pdf:  samples/sample-xelatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && xelatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && xelatex-dev $(notdir $<)
	cd $(dir $@) && xelatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && xelatex-dev $(notdir $<); done

samples/sample-lualatex.pdf:  samples/sample-lualatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && lualatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && lualatex-dev $(notdir $<)
	cd $(dir $@) && lualatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && lualatex-dev $(notdir $<); done

samples/sample-acmcp.pdf: samples/acm-jdslogo.png

.PRECIOUS:  $(PACKAGE).cfg $(PACKAGE).cls

docclean:
	$(RM)  *.log *.aux \
	*.cfg *.glo *.idx *.toc \
	*.ilg *.ind *.out *.lof \
	*.lot *.bbl *.blg *.gls *.cut *.hd \
	*.dvi *.ps *.thm *.tgz *.zip *.rpi \
	samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst \
	samples/*.log samples/*.aux samples/*.out \
	samples/*.bbl samples/*.blg samples/*.cut \
	samples/acm-jdslogo.png \
	samples/*.run.xml samples/*.bcf $(SAMPLEBIBLATEXFILES)


clean: docclean
	$(RM)  $(PACKAGE).cls \
	samples/*.tex

distclean: clean
	$(RM)  *.pdf samples/sample-*.pdf

#
# Archive for the distribution. Includes typeset documentation
#
archive:  all clean
	COPYFILE_DISABLE=1 tar -C .. -czvf ../$(PACKAGE).tgz --exclude '*~' --exclude '*.tgz' --exclude '*.zip'  --exclude CVS --exclude '.git*' $(PACKAGE); mv ../$(PACKAGE).tgz .

zip:  all clean
	zip -r  $(PACKAGE).zip * -x '*~' -x '*.tgz' -x '*.zip' -x CVS -x 'CVS/*'

# distros
distros: all docclean
	zip -r acm-distro.zip  \
	acmart.pdf acmguide.pdf samples *.cls ACM-Reference-Format.* \
	--exclude samples/sample-acmengage*
	zip -r acmengage-distro.zip samples/sample-acmengage* \
	samples/*.bib \
	acmart.pdf acmguide.pdf  *.cls ACM-Reference-Format.*


.PHONY: all ALLSAMPLES docclean clean distclean archive zip


==> README <==
This package provides a class for typesetting publications of the
Association for Computing Machinery.

Your TeX distribution probably includes the latest released version of
this package.  If you decide to install it yourself, please see the
Installation section of the User's Guide.

Please note that the version on Github is a development (or
experimental) version: please download it for testing new features.
The production version is the one on CTAN and ACM sites.


Changes

Version 1.90   Journal ISSN updated

Version 1.89a  Added version info to .bst

Version 1.89   Bug fixes
	       Redesign of ACMCP
	       New positioning of badges
	       New journals: PACMMOD, TOPML

Version 1.88   New ISSNs
	       Documentation updates
	       New journal:  PACMNET

Version 1.87   CC license is allowed for non-acm documents and ACM Engage
	       documents only
	       New format acmcp for the cover page
	       New journals: JATS, ACMJCSS, TORS
	       Bug fixes

Version 1.86.  Empty country in affiliation now produces an error
               Bug fixes
	       New samples for acmengage

Version 1.85.  Bug fixes
	       Added support for Creative Commons licenses (requires
	       doclicense images)
	       New journals
	       New format acmengage for ACM Engage CSEdu course materials 

Version 1.84   Support for BibLaTeX rewritten (thanks to
	       Roberto Di Cosmo and Kartik Singhal)
	       Corrected German translation (thanks to Dirk Beyer)
	       New journals

Version 1.83   Support for multilanguage papers
	       ISSN changes for some journals

Version 1.82   Bug fixes.
	       New command \anon for anonymization of short strings.
	       Documentation update.

Version 1.81   Bug fixes
	       New bib field distinctURL to print URL even if doi is present.
	       Reworded samples

Version 1.80   New journals: DLT, FAC

Version 1.79   Fixed pages with index
	       (https://github.com/borisveytsman/acmart/issues/440)
	       Updated information for TAP, TCPS, TEAC

Version 1.78   Documentation update.
	       Magic texcount comments for samples.
	       Title page now is split if there are too many authors
	       Bug fixes.

Version 1.77   Changed the way to typeset multiple affiliations (Christoph Sommer)

Version 1.76   Added many journal abbreviations to the bst.
	       New experimental option: pbalance
	       ORCID linking code

Version 1.75   Omitted \country now produces error.
	       Added \AtBeginMaketitle

Version 1.74   Bug fixes.  A regression introduced in the font changes
	       is reverted.

Version 1.73   Bug fixes
	       The elements institution, city and country are now obligatory
	       for affiliations.  The absence of them produces a warning

Version 1.72   Bug fixes.  Better handling of metadata.

Version 1.71   Bug fixes
               Formats sigchi and sigchi-a are retired
	       Bibliography formatting changes for @inproceedings entries
	       having both series and volume
	       LuaLaTeX now uses the same OTF fonts as XeLaTeX

Version 1.70   Title change for ACM/IMS Transactions on Data Science
               Bug fixes for bibliography

Version 1.69   Bug fixes
	       Compatibility with LaTeX 2020-02-02 release

Version 1.68   Bug fixes
               BST now recognizes words `Paper' or 'Article' in
	       eid or articleno

Version 1.67   Urgent bug fixes:
	       BibTeX style bug fixed (Michael D. Adams)
	       Sigplan special section bugfix

Version 1.66   Bug fixes
	       BibTeX change:  location is now a synonym for city (Feras Saad) 
	       ACM reference format is now mandatory for papers over one page.
	       CCS concepts and keywords are now mandatory for
	       papers over two pages.
	       Authors' addresses are mandatory for journal articles.

Version 1.65   Bug fixes
	       New journal: DGOV
	       DTRAP and HEALTH are now using acmlarge format

Version 1.64    Produce error if abstract is entered after maketitle
		(previously abstract was silently dropped)
		Bug fixes for line numbering

Version 1.63a   Moved TQUANT to TQC

Version 1.63	New journals: TQUANT, FACMP

Version 1.62    Documentation update
		New journal: TELO
		Bug fixes

Version 1.61    Bug fixes
                New bibtex types for artifacts

Version 1.60    New option: urlbreakonhyphens (thanks to Peter Kemp)
		Smaller header size for acmsmall

Version 1.59    Now a journal format can be used for conference proceedings
		All samples are now generated from the same .dtx file
		Bug fixes

Version 1.58    Suppressed spurious warnings.
		New journal:  HEALTH.
		TDSCI is renamed to TDS.

Version 1.57    Change of \baselinestretch now produces an error
                Booktabs is now always loaded
                Added option `balance' to balance last page in two-column mode
                E-mail is no longer split in addresses
                New samples (Stephen Spencer)

Version 1.56    Bug fixes
                Added \flushbottom to two column formats (Philip Quinn)
                The final punctuation for the list of concepts
                is now a period instead of a semicolon (Philip Quinn)
                New command \Description to describe images for visually
                impaired users.

Version 1.55    Bug fixes
                Font changes for SIGCHI table captions

Version 1.54    New option: 'nonacm' (Gabriel Scherer)
                Deleted indent for subsubsection (suggested by Ross Moore)
                Suppressed some obscurious warning in BibTeX processing
                Suppressed hyperrerf warnings (Paolo G. Giarrusso)
                New code for sections to help with accessibility patches
                (Ross Moore)
                Submission id, if present, is printed in anon mode
                Bug fixes

Version 1.53    New journals: PACMCGIT, TIOT, TDSCI

Version 1.52    Another rewording of licenses

Version 1.51    Journal footers now use abbreviated journal titles.
                Corrected the bug with acmPrice.
                Do not show price when copyright is set to iw3c2w3 and iw3c2w3g.
                The package now is compatible with polyglossia (Joachim Breitner).
                Slightly reworded copyright statements.

Version 1.50    Changes in iw3c2w3 and iw3c2w3g

Version 1.49    New jorunal:  DTRAP

Version 1.48    Bug fixes
                Review mode now switches on folios
                Code prettying (Michael D. Adams)
                Bibliography changes: @MISC entries no longer have a
                separate date
                Sigch-a sample bibliography renamed
                Bib code cleanup (Zack Weinberg)
                Acmart and version info are added to pdfcreator tag
                \citeyear no longer produces parenthetical year
                Added initial support for Biblatex (Daniel Thomas)
                Added support for IW3C2 conferences

Version 1.47    New journal: THRI

Version 1.46    Bug fixes for bibliography: label width is now calculated
                correctly.
                All PACM now use screen option.  This requires etoolbox.
                Added subtitle to ACM reference format.
                Now acmart is compatible with fontspec.
                \thanks is now obsolete.  The addresses are automatically
                added to the journal version; this can be overriden with
                \authorsaddresses command.
                Deleted the rule at the end of frontmatter for all formats.
                Deleted new line before doi in the reference format.
                Reintegrated theorem code into acmart.dtx (Matthew Fluet)

Version 1.45    Workaround for a Libertine bug.  Thanks to LianTze Lim
                from Overleaf

Version 1.44    Bug fixes.
                Empty DOI and ISBN suppress printing DOI or ISBN lines
                Separated theorem code into acmthm.sty, loaded by default.
                Article number can be set for proceedings.
                New commands: \acmBooktile, \editor.
                Reference citation format updated.

Version 1.43    Bug fixes

Version 1.42    Deleted ACM badges
                Bug fixes

Version 1.41    Rearranged bib files
                Added new badges

Version 1.40    Bibliography changes
                Added processing of one-compoment ccsdesc nodes
                Bug fixes.
                Made the height a multiple of \baselineskip + \topskip
                Added cleveref
                We no longer print street address in SIGs

Version 1.39    Added \authornotemark commmand

Version 1.38    Increase default font size for SIGPLAN

Version 1.37    Reduce list indentation (Matthew Fluet)

Version 1.36    Bug fixes
                Moved PACMPL to acmlarge format
                New journal: PACMHCI
                Added the possibility to adjust number of author
                boxes per row in conference formats

Version 1.35    Author-year bib style now uses square brackets.
                Changed defaults for TOG sample
                Price is suppressed for usgov and rightsretained modes.
                Bugs fixed

Version 1.34    Deleted DOI from doi numbers
                Changed bibstrip formatting
                The command \terms is now obsolete
                The rulers in review mode now have continuous numbering

Version 1.33    New option `timestamp' (Michael D. Adams)
                New option `authordraft'
                Documentation updates
                Bug fixes
                We now use Type 1 versions of Libertine fonts even with XeTeX.
                New hook acmart-preload-hook.tex (wizards only!)
                Added new options `obeypunctuation' for \affiliation command
                Added SubmissionID
                Added right line count ruler for two-column formats
                Added workaround for Adobe Acrobat bugs in selection
                Added eid field to the bibliography

Version 1.32    New DOI formatting.
                Format siggraph is now obsolete, and sigconf
                is used instead.
                New proceedings title: POMACS.

Version 1.31    Changed default year and month to the current ones
                (thanks to Matteo Riondato)
                Table of contents now works
                Marginalia now work in all formats
                New command \additionalaffiliation
                Documentation changes

Version 1.30    Bibtex style now recognizes https:// in doi.
                Added \frenchspacing.
                \department now has an optional hierarchy level.
                Switched to T1 encoding
                Updated IMWUT and PACMPL

Version 1.29    Documentation changes.  Head height increased from 12pt to 13pt.
                Removed spurious indent at start of abstract.
                Improved kerning in CCS description list.

Version 1.28    Bug fixes: natbib=false now behaves correctly.

Version 1.27    Bug fixes

Version 1.26    Bug fixes

Version 1.25    Updated PACMPL journal option.

Version 1.24    Added IMWUT journal option.

Version 1.23    Added PACM PL journal option.

Version 1.22    Bibliography changes for Aptara backend; should be
                invisible for the users.

Version 1.21    Bibliography changes: added arXiv, some cleanup

Version 1.20    Bug fixes, documentation updates

Version 1.19    Include 'Abstract', 'Acknowledgements', and 'References'
                in PDF bookmarks.

Version 1.18    Natbib is now the default for all versions.  A unified bib
                file is used for all styles.  Better treatment
                of multiple affiliations.


Version 1.17    Formatting changes for margins and lists.  Bug fixes.

Version 1.16    Formatting changes for headers and footers.

Version 1.15    New structured affiliation command.
                New commands for acknowledgements.

Version 1.14    Warn about undefined citation styles; move definitions
                of acmauthoryear and acmnumeric citation styles before
                use.

Version 1.13    Formatting changes: headers, folios etc.
                Bibliography changes.

Version 1.12    Bug fixes and documentation updates.
                Footnotes rearranged.
                Option natbib is now mostly superfluous: the class
                makes a guess based on the format chosen.

Version 1.11    Customization of ACM theorem styles and proof
                environment (Matthew Fluet).

Version 1.10    Bug fixes

Version 1.09    SIGPLAN: revert caption rules (Matthew Fluet)

Version 1.08    SIGPLAN reformatting (Matthew Fluet); bug fixes


==> archived/Xdonotedit-intro-old.tex <==
\section{Introduction}

Generative Pre-trained Transformer (GPT) language models~\cite{radford:gpt2:2019} can \add{assist in data-driven knowledge work} \del{analyze and visualize data} by producing \del{and executing} code outputs from natural language inputs~\cite{Feng:CodeBert:2020,Austin:ProgramSynth:2021,Poesia:Synchromesh:2022}. These capabilities can support novice and expert analysts alike by reducing barriers \add{around conducting}\del{and the effort required to conduct} \del{at least} preliminary investigations of data~\cite{Maddigan:Chat2Vis:2023,Dibia:LIDA:3034,cheng:llm_analyst:2023}, \add{including transforming and visualizing multidimensional datasets}. \del{Although promising, these} These models do not reflect the first attempt to scaffold data analysis through visual and naturalistic interfaces.  Prior research on Visual Natural Language Interfaces (V-NLIs) and conversational agents have explored varying techniques\del{,} from heuristics to alternative deep learning models\del{,} for translating plain language utterances into corresponding data transformations and visualization specifications~\cite{Hoque:ChartQAStar:2022,Shen:NLISurvey:2023,mctear:conversational_agent:2022,voigt:VNLISurvey:2022,Srinivasan:NLI:2017}. In addition to delineating a design space for V-NLIs, these prior efforts also document the multi-faceted and dynamic nature of analytic conversations.


% It has yet to be assessed how GPT language models function as part of V-NLIs, including conversational interfaces, and how they respond to the nuanced characteristics of analytic conversations. These include the ambiguity and intents of individual utterances~\cite{Srinivasan:Snowy:2021,setlur:eviza:2016}, the role of language pragmatics and context in generating appropriate data transformations and visual specifications~\cite{Hoque:Evizeon:2018}, and the multi-step operations required to produce a desired output~\cite{Fast:Iris:2019}. 
A recent head-to-head comparison of GPT language models and several V-NLIs suggests that GPT performance is as capable, and potentially superior, to prior systems for the first conversational characteristic~\cite{Maddigan:Chat2Vis:2023}. The capacity of GPT language models to carry out multi-step analytic operations, a documented weakness~\cite{Dziri:Compositionality:2023}, was not explicitly evaluated. Moreover, this assessment focused on individual utterances and did not consider shifting conversational context that accompanies the refinement of analysis questions and visual outputs~\cite{Fast:Iris:2019,tory:tc17:2019}. It also remains to be determined whether GPT language models maintain appropriate coherence~\cite{tory:tc17:2019} in light of evolving conversations. 

We conduct a deeper investigation into a GPT model's ability to carry out visual analytic conversations. Our research has two parts. In the first part, we develop an interface that uses a GPT language model as a conversational agent to produce both visual and textual outputs in response to user utterances. We describe how we augment these utterances with prompt templates to overcome token limitations and improve the reliability of agent's responses. We also describe a novel multi-threaded approach for managing conversational context to the GPT agent that improves the coherence of visual outputs. We use tasks from prior V-NLI systems to evaluate our interface. In the second part, we conduct two usability studies to assess the validity, robustness, and utility of our conversational agent. The first is a crowd-sourced study with XX participants, followed by a second in-depth study that conducted semi-structured interviews with XX participants. The findings from these user studies show that participants had an overall positive perception of the our agent's outputs and were often delighted by the ease of analyzing data. Participants also point to several areas where out agent could further improve to better support their analysis objectives. Collectively, we present four research contributions:

Our primary contributions are:
\begin{itemize}
    \item An evaluation of a generative pre-trained transformer (GPT) language model for conducting a data analysis with shifting conversational context
    \item The design of multithreaded analytic conversations and their applications to GPT models.
    \item The~\sysname~interface for conducting threaded analytic conversations using GPT-models.
    \item The results of a user study that showcases both the capabilities and limitations of GPT language models as analytic conversational agents 
\end{itemize}

Conversational agents supported by GPT language models are poised to play a larger role in data analysis, including the generation of visualizations. Our research presents a novel approach to supporting these complex and multi-faceted conversations. 


----


\section{Introduction}

Generative Pre-trained Transformer (GPT) language models~\cite{radford:gpt2:2019} can \add{assist in data-driven knowledge work} \del{analyze and visualize data} by producing \del{and executing} code outputs from natural language inputs~\cite{Feng:CodeBert:2020,Austin:ProgramSynth:2021,Poesia:Synchromesh:2022}. These capabilities can support novice and expert analysts alike by reducing barriers \add{around conducting}\del{and the effort required to conduct} \del{at least} preliminary investigations of data~\cite{Maddigan:Chat2Vis:2023,Dibia:LIDA:3034,cheng:llm_analyst:2023}, \add{including transforming and visualizing multidimensional datasets}. \del{Although promising, these} \del{These models do not reflect the first attempt to scaffold data analysis through visual and naturalistic interfaces} Prior research on Visual Natural Language Interfaces (V-NLIs) and conversational agents have explored varying techniques\del{,} from heuristics to alternative deep learning models\del{,} for translating plain language utterances into corresponding data transformations and visualization specifications~\cite{Hoque:ChartQAStar:2022,Shen:NLISurvey:2023,mctear:conversational_agent:2022,voigt:VNLISurvey:2022,Srinivasan:NLI:2017}.
\add{System capabilities of this prior research may be subsumed into the emergent properties of GPT models}. 
% It has yet to be assessed how GPT language models function as part of V-NLIs, including conversational interfaces, 
% and how they respond to the nuanced characteristics of analytic conversations. These include the ambiguity and intents of individual utterances~\cite{Srinivasan:Snowy:2021,setlur:eviza:2016}, the role of language pragmatics and context in generating appropriate data transformations and visual specifications~\cite{Hoque:Evizeon:2018}, and the multi-step operations required to produce a desired output~\cite{Fast:Iris:2019}. 
A recent head-to-head comparison of GPT language models and several V-NLIs suggests that GPT performance is as capable, and potentially superior, to prior systems for \del{the first conversational characteristic}\add{resolving ambiguities around user intent behind an utterance}~\cite{Maddigan:Chat2Vis:2023}. 

It has yet to be assessed how GPT language models function as part of V-NLIs, including conversational interfaces. Rather than focusing on individual utterances, \add{our work considers} the shifting conversational context that accompanies the refinement of analysis questions and visual outputs~\cite{Fast:Iris:2019,tory:tc17:2019} \add{given} the multi-step operations required to produce a desired output~\cite{Fast:Iris:2019}.
\add{Most utterances do not produce pertinent data artifacts, but simply transition from a preliminary state toward an insightful visualization~\cite{tory:tc17:2019}.}
In light of this observation, we \add{developed a conversational visualization interface powered by GPT} to conduct a deeper investigation into \del{a GPT model's} \add{its} ability to carry out \del{visual analytic conversations}\add{conversational data analysis}, \add{specifically focusing on the requirement that conversational agents need to} maintain \textit{coherence}~\cite{tory:tc17:2019} in light of evolving data conversations.
\add{Our goal is to study} the ambiguity and intents of individual utterances~\cite{Srinivasan:Snowy:2021,setlur:eviza:2016} and the role of language pragmatics and context in generating appropriate data transformations and visual specifications~\cite{Hoque:Evizeon:2018} \add{when a foundational model is integrated into a conversational workflow.}
\del{The capacity of GPT language models to carry out multi-step analytic operations, a documented weakness~\cite{Dziri:Compositionality:2023}, was not explicitly evaluated.}
% Moreover, this assessment focused on individual utterances and did not consider shifting conversational context that accompanies the refinement of analysis questions and visual outputs~\cite{Fast:Iris:2019,tory:tc17:2019}. 
% It also remains to be determined whether GPT language models maintain appropriate coherence~\cite{tory:tc17:2019} in light of evolving conversations. 
% We conduct a deeper investigation into a GPT model's ability to carry out visual analytic conversations. 

Our research has two parts. We first develop an interface that uses a GPT language model as a conversational agent to produce both visual and textual outputs in response to user utterances \add{while incorporating a common feature of messaging apps---the ability to reply to and continue a conversation inside a thread---}for \del{managing conversational context to the GPT agent}\add{an analyst to manage context}  \del{that improves the coherence of visual outputs}\add{to improve conversational coherence.} In the second part, \add{we use tasks from prior V-NLI systems to conduct} two usability studies to assess the validity, robustness, and utility of our conversational agent. The first is a crowd-sourced study with XX \add{novice} participants, followed by a second in-depth study that conducted semi-structured interviews with XX \add{expert} participants. The findings from these user studies show that participants had an overall positive perception of the our agent's outputs and were often delighted by the ease of analyzing data. \add{Expert} participants also \add{ideated} \del{pointed to} several areas \add{of future work} \add{with regards to the capabilities of GPT-supported conversational visual analysis software} \del{could further improve} to better support their analysis \add{needs}\del{objectives}. Collectively, we present three research contributions:

Our primary contributions are:
\begin{itemize}
    \item The design of multithreaded analytic conversations and their applications to GPT models.
    \item The~\sysname~interface for conducting threaded analytic conversations using GPT-models.
    \item The results of a user study that showcases both the capabilities and limitations of GPT language models as analytic conversational agents 
\end{itemize}

Conversational agents supported by GPT language models are poised to play a larger role in data analysis, including the generation of visualizations. Our research presents a novel approach to supporting these complex and multi-faceted conversations. 

==> archived/related_work_old.tex <==
\section{Related Work}\label{rw}
We summarize related work pertinent to Visual natural Language Interfaces, Conversational agents, and visualization recommendation systems. 

%=========================
% V-NLIs
%=========================
\subsection{Visual Natural Language Interfaces (V-NLIs)}\label{rw:nli}
 
 
 The ways that different NLI systems go about these tasks can be broken down into three primary approaches, symbolic, deep learning, and more recently generative pre-trained transformer (GPT)~\cite{Maddigan:Chat2Vis:2023,Shen:NLISurvey:2023}.

Symbolic approaches to V-NLIs use explicit structures, such as parse trees, grammars, heuristics, and rule-base approaches to parse a natural language query and determine the appropriate output. Examples of such systems include DataTone~\cite{Gao:DataTone:2015}, Eviza~\cite{setlur:eviza:2016}, and FlowSense~\cite{Yu:FlowSense:2020}. These early approaches also uncovered a number of challenges, and propose initial solutions, pertaining to the under-specification queries and language ambiguities, as well as issues of conversational coherence and context (pragmatics). Evizeon~\cite{Hoque:Evizeon:2018} further explored the concept of pragmatics to maintain coherence in visual analytic conversations by augmenting the state transition model used in the Eviza systems~\cite{setlur:eviza:2016}.  The Orko~\cite{Srinivasan:orko:2018} applies these concepts to networks; it is one of the few examples that demonstrates these concepts on non-tabular datasets. While symbolic approaches perform reasonably well and are reasonably transparent, they can also suffer from brittleness that limits their efficacy~\cite{Maddigan:Chat2Vis:2023}.

Deep Neural Network (DNN) approaches for V-NLIs try to learn an association between data, natural language queries, and target visualization. The goal of these approaches is to learn a possible mapping function between the inputs (Data and Utterances) and outputs (Visualizations) without having to explicitly specify this function, as it is done in symbolic approaches. Examples for such systems include, Advisor~\cite{Liu:ADVISor:2021}, ncNet~\cite{Yuyu:ncNet:2022}, Talk2Data~\cite{Guo:Talk2Data:2021},  and Urania~\cite{Guo:Urania:2023}. These DNN approaches vary on the specific architecture they employ to learn these mapping functions. For example, ncNet uses an encoder-decoder transformer model, whereas Urania bidirectional LSTM to learn the association between data, questions, and visualization schemas.  One of the limitations of these approaches is that they can require large annotated datasets, which are often difficult to obtain. 

With the capacity got GPT models to generate programs improving~\cite{Austin:ProgramSynth:2021}, more recent research has also begun to investigate these approaches to support V-NLIs. Chat2Vis~\cite{Maddigan:Chat2Vis:2023} uses GPT-3.5, as do we, to generate visualizations from natural language queries of a dataset.  Unlike DNN approaches, GPT models do not require an additional labelled dataset to produce visualization recommendations and would require minimal data if fine-tuning were desirable~\cite{Brown:LLM_fewshot:2020}. Indeed Maddigan~\textit{et. al.}~\cite{Maddigan:Chat2Vis:2023} find this to be the case when the compare they compare their GPT approach to symbolic and DNN approaches in six tasks. Our research extends the exploration of GPT-based approaches from Chat2Vis and addresses several of the outstanding challenges they identified.

The overall trajectory of underlay technology that supports V-NLIs mirrors the evolution of many other domains, such as image recognition or text generation, that similarly began with the explication of model or heuristic, followed by the use of Neural Networks, and more recently the use of GPT. All of these approaches have their strengths and limitations. In our research, we further investigate the use of GPT approaches for V-NLI. We consider many of the concepts explored in prior systems, particularly coherence, in our system design and evaluation.


%=========================
% Conversational Agents
%=========================
\subsection{Conversational Agents for Visual Data Analysis}

Conversational agents are dialogue systems, typically deployed as chatbots, that facilitate a naturalistic conversational flow between a person conducting the analysis and an automated agent~\cite{mctear:conversational_agent:2022}. Chatbots that produce visualizations are a subset of the V-NLI design space and utilize many of the techniques that support V-NLIs and also visualization recommendation~\cite{Kavax:ChatvNLI:2023,Setlur:gricean_maxims:2022}. Both designs of chatbot interfaces and the structure of analytic conversations are pertinent prior art to our research, and as such, we focus on this topic in more depth that V-NLIs in general. 

Prior research has used various approaches to study to analytic conversations with chatbots. There is prior precedence in chatbots as being primarily text-based interactions, with text responses. Hearst and Tory~\cite{Hearst:ChartChat:2019} show that this influences expectations when conversing with these bots, with participants sometimes showing a greater preference for text responses over visualizations. Setlur and Tory~\cite{tory:tc17:2019} use a wizard-of-oz study to study the relationship between participant utterances and the automatic generation of visualizations. Their study consists of four conditions, including two that incorporate context, and that explore the evolving structure of analytic conservation. They summarize their findings as a state transition model and discuss the importance of context and intent to facilitate these transitions and support both conversational and visual coherence. In follow-up research, they also demonstrate the importance of the input medium and modalities (voice or text) in influencing these conversations~\cite{Setlur:gricean_maxims:2022}. They found that text interactions in combination with conversational threading supported a deeper analysis compared to other modalities.

A small number of systems have been implemented that support analytic conversations with text interfaces. Iris~\cite{Fast:Iris:2019} is intended to support data science applications and outputs either a text or visual response. Their prototyping focus on the combination of utterances to produce an appropriate response. Kim~\textit{et. al.}~\cite{Kim:ChatQA:2020} implement a pipeline that leverages natural language templates to facilitate a conversation for explaining visualizations.  Both~\cite{Fast:Iris:2019} and~\cite{Kim:ChatQA:2020} touch upon the importance of composition operations (i.e. requiring multiple operations) to carry out these analytic conversations. Recent research has shown that GPT models can struggle with compositional tasks~\cite{Dziri:Compositionality:2023}; we examine this in our research. Finally, to support participants in visual analysis, SNOWY~\cite{Srinivasan:Snowy:2021} produces ranked suggestions for utterances that users may pose of the data and visualization. 

Collectively, this research is a space of techniques and design principles that we leverage and extend in our research. We extend the ideas of conversational threading to GPT models and further explore issues of coherence and compositionality.


%=========================
% Vis Recommendations
%=========================
\subsection{Visualization Recommendation}\label{rw:vizrec}
Visualization recommendation (VisRec) techniques attempt to automatically generate visualizations primarily based on the attributes of the data. While VisRec techniques need not be tied specifically to NLI inputs, they can be considered a complementary approach to generating visualizations it varying degrees of input specification.  Similarly to V-NLIs, there exist varying approaches to recommending visualizations. 

ShowMe~\cite{Mackinlay:ShowMe:2007} uses a rule-based approach predicated on the field types (categorical or numeric) and best practices ranking. It requires the use to specify one or more fields before it can automatically generate an encoding. VizDeck~\cite{Key:VizDeck:2012} similarly used data properties to recommend interactive dashboards, instead of single encodings. ShowMe was further extended in the Voyager and Voyager2 systems~\cite{Wongsuphasawat:Voyager:2016}, which use statistical properties of the dataset to automatically generate and rank visualizations of a dataset while relaxing the requirement of an initial user specification. The Voyager systems almost recommend multiple encodings that users can bookmark visualizations they find interesting to revisit later. Finally, Draco~\cite{Moritiz:Draco:2019} presented an approach to automatically incorporate perceptual efficacy experiments into these visualization recommendation paradigms. 

More recent techniques for visualization recommendation incorporate information about the analysis task, user intent, or application domain. TaskVis~\cite{Agus:TaskVis:2021} uses a pre-defined set of tasks and rule-based approach to recommend visualization from a combination of data fields and analytic tasks. Frontier~\cite{Lee:Frontier:2022} similarly uses pre-defined task and intent classifications for data analysis to generate and organize visualization recommendations. The concepts of Frontier are reified in the Lux~\cite{Lee:Lux:2021}, a Jupyter notebook widget that interacts with Pandas, a widely used Python data analysis library. Medely extends these intent-based recommendations further to generate dashboard visualizations~\cite{Pandey:Medely:2023}. ChartSeer~\cite{Zhao:ChartSeer:2022},Chart2Vec~\cite{Chen:Chart2Vec:2023} and DeepEye~\cite{Luo:DeepEye:2018} propose machine learning approaches as alternatives to the rule-based methods.  Both ChartSeer~\cite{Zhao:ChartSeer:2022} and Chart2Vec~\cite{Chen:Chart2Vec:2023} learning a vector representation of visual encodings, albeit in different ways, to recommend visualizations, while DeepEye~\cite{Luo:DeepEye:2018} uses a learning-to-rank approach. Recently, LIDA was developed as way to recommend visualizations by using a GPT approach to generate specifications~\cite{Dibia:LIDA:3034}. 

Finally, visualization recommendations can also take domain context into account. For example, GenoRec~\cite{Pandey:GenoRec:2023} and GEViTRec~\cite{Crisan:GEviTREc:2022} both leverage data from the genomics domain to generate recommendations.

The primary difference between these existing approaches to data visualization recommendations and those created by LLMs is the level of specificity of the user. In all of these existing visualizations, the user needs to explicitly specify data fields, tasks, intents, and/or domain context to generate recommendations. In contrast, LLMs largely infer these specifications from a natural language prompt. In this research, we investigate both the quality of the LLM response and the level of specificity of the natural prompt that is required to produce a satisfactory visualization. 


%=========================
% Prompt Engineering
%=========================

%\subsection{Prompt Engineering Strategies and Tools}\label{rw:pe}
%\ana{Maybe this doesn't need to be here, but I'll leave it here for now}
%GPT-based approaches rely on effective prompts to generate quality results~\cite{Brown:LLM_fewshot:2020}. Recent research has explored approaches and tooling for supporting effective prompt creation. AI Chains~\cite{Wu:LLM_chains:2022} proposes several primitive operations for prompt engineering; their approach creates a chain of prompts breakdown the original prompt into a set of subtasks to refine LLMs output. The advantage this approach, besides improving the model's response, is that it makes the prompt both more transparent and debuggable.  Its often necessary to explore a variety of prompting strategies. This exploration can be done automatically~\cite{Zhou:APE:2022} or through manual means that allow users to explore different prompt templates, visualize there results, and iterate~\cite{Storbel:PEngVis:2023,Mishra:PromptAid:2023,Singh:ExplainingPE:2022}. We do not expose prompt engineering available in our system, but, use the strategies from these prior works to develop an appropriate instructional prompt that augments the user's natural language queries.\











==> tex/Xinterface_design.tex <==
\section{\sysname}\label{interface}
For the analyst, our goal is to create a conversational user interface while supporting the non-linear nature of visual data analysis.
The main interface of \sysname comprises the Main Chat and Thread components, akin to instant messaging apps which allow users to start threaded conversations within messages and keep discussions organized.
Users can upload their own datasets, and visualizations are displayed as static images rendered with Seaborn accompanied by relevant alt-text captions that ensure accessibility and support communication of insights.
Further augmenting the system are the Data Dictionary and embodiments for revising or rectifying LLM outputs.

\subsection{Persistent Data Dictionary}
To reduce the need for users to repeatedly recall the structure of their dataset in the design of analytic prompts, \sysname keeps pertinent information about data columns at the bottom of the chatbot interface.
As will be described in the next section, the ``Description'' row is populated by the LLM.
However, users can edit it if the LLM's descriptions are inaccurate.
Editing the description row facilitates natural language interaction by helping the LLM understand ambiguous data semantics.

\subsection{The Main Chat and Thread}
A clear advantage of chatbots for visual data analysis is that a conversational workflow supports a progressive and inductive sensemaking process over the collected dataset, without requiring the user or the AI to have command over the data set a priori.
Users obtain visualizations of data through natural language prompts in the Main Chat by asking questions or issuing commands.
The insights produced by these visualizations can be used to inform subsequent analytic prompts.

However, given an ambiguous prompt (such as ``age
vs surviving'') that lacks specificity about visualization tasks or chart types, the AI's answers may not be insightful (Figure 1).
Threads are used to refine and customize visualizations.
In a Thread, users might modify visual encodings to experiment with different chart configurations.
Users can also disaggregate or aggregate a column if the LLM has made dissatisfactory calculations in its attempt to infer user intent.
As an example, one misalignment may be the LLM binning a histogram in steps too narrow for any insightful data pattern to emerge.
The LLM may also infer that the user wanted an aggregated rate across a count (e.g., the number of male survivors vs. survival rate among men) and such assumptions may not be desirable.
Lastly, it may be that the user has entered a prompt lacking in specificity, but the LLM may still output a response that only needs a few adjustments to be insightful.
In summary, misalignments that may need correction inside a Thread may arise from:

\begin{enumerate}
  \item degrees of freedom inherent to the design of clear data visualizations;
  \item the LLM making assumptions without a clear understanding of the user's intent; or
  \item the user's lack of specificity in their prompts in the absence of a priori empirical knowledge, which can only emerge from the generation of visualizations.
\end{enumerate}

Users may also experiment with adding annotations, adding reference and regression lines, or making aesthetic changes.
Once a Thread is exited, the last visualization in the Thread replaces the original iteration within the Main Chat.

The resulting conversation in the Main Chat serves as a notebook-style data artefact to be shared as well as a trail of the user's analytic process, although the user may open the thread to reveal deeper provenance of how they arrived at the data insights.
Toward this goal, \sysname can maintain coherence and a sense of continuity in the Main Chat without detailed refinements disrupting the exploration and communication phases of data analysis.

\subsection{Prompt Revisions}
\sysname enables an effective analytic workflow by offering intuitive ways to correct errors or experiment with different prompts when interfacing with the stochastic outputs of LLMs.
In both the Main Chat and the Thread, unexpected outcomes can be backtracked or rectified with either the “Redo” or the "Undo" feature.
Users can hit the “Redo” button to request a new response to an analytic prompt; \sysname stores each previous version of the response as a safety net to avoid losing previous outcomes by accident, or if the user decides they prefer a previous version.
Users can also prompt the system to “undo” the user’s last prompt, which allows users to wholly revise their instructions if they realize their prompt cannot be effectively answered by the data and the AI, leading to a dead end.



==> tex/xsystem_design.tex <==
\section{System Design}
Data Threads uses the GPT-3.5 model through OpenAI’s ChatCompletion API to generate visualizations based on descriptions of the dataset and users' visualization queries.
As a successor to both GPT-3 and Codex models, GPT-3.5 may be capable of visualization code synthesis from user prompts even when there are ambiguities in user intent.
We utilized instructional system prompts and examples for the model to generate valid visualization code using Python libraries \texttt{pandas} and \texttt{seaborn} which enable efficient data manipulation, processing, and visualization rendering.

\subsection{Creating the Dataset Dictionary}
\label{sec:dictionary}
An ``uploaded" dataset is simply stored as a string referring to the file's location in the local filesystem, which the synthesized code will use to indirectly perform data manipulation.
Since the LLM does not have direct access to the dataset, it is important to provide the model with a dataset dictionary that contains pertinent information such as a field's data type and its range (for quantitative data) or an exemplar (for qualitative data). 
The model will also require a natural language description of the field in order to understand the user's intent in cases where the user does not refer to a field by its exact name. 
When a dataset is uploaded, its column names and Pythonic data types are extracted using \texttt{pandas}.
For quantitative fields, their minimum and maximum values are also extracted; for qualitative fields, their first non-null row values are extracted instead.
The resulting but preliminary data dictionary as a markdown table is input to Algorithm \ref{alg:dictionary-chain}, which describes the prompt given to GPT-3.5 to produce the full dictionary.

\begin{center}
\noindent
\shadowbox{%
  \begin{minipage}{0.94\linewidth}
    Computations described in \S\ref{sec:dictionary} using \texttt{pandas} will produce a markdown table with the following columns:

    \begin{lstlisting}
|            | Data Type  | Range or Example       |
|:-----------|:-----------|:-----------------------|
    \end{lstlisting}

    Given this table, the final step of the data uploading stage involves querying an LLM to produce natural language descriptions for the dataset fields. 
    We first instruct GPT-3.5 with the following system prompt:

    \begin{lstlisting}
We will generate markdown tables that begin with the following columns:
|            | Data Type  | Range or Example       | Description               |
|:-----------|:-----------|:-----------------------|:--------------------------| 
    \end{lstlisting}

    And finally request an output with the following prompt:
\begin{lstlisting}
Here is a markdown table summarizing columns in [FILENAME]:
[ORIGINAL TABLE]
Generate descriptions for what the data column values mean and concatenate the descriptions to the markdown table.
\end{lstlisting}
  \end{minipage}%
}
\captionof{algorithm}{Your caption here.}
\label{alg:dictionary-chain}
\end{center}

As described earlier, the Data Threads interface also displays this table for the user and allows them to modify the description of a field when the LLM cannot infer it correctly from the column names and examples alone.

\subsection{Generating a Chart}
Once a user inputs a query prompt, Data Threads performs several computations before rendering a chart image.

\subsubsection{Prompt Augmentation} 
System instruction prompts that define an LLM's \textbf{\textcolor[RGB]{117, 112, 179}{role}} and \textbf{\textcolor[RGB]{27, 158, 119}{desired behaviors}} can augment user prompts to better align its responses.
Before a user's analytic prompt is sent to the GPT-3.5 ChatCompletion API, which conversation and instruction prompt are sent with it varies depending on whether the user is interfacing with the Main Chat or a Thread:



\paragraph{Instructions in the Main Chat}

\texttt{\textcolor[RGB]{117, 112, 179}{You are a data visualization assistant working with a dataset called [FILENAME]. You will answer questions with this dataset.}} 
\texttt{\textcolor[RGB]{27, 158, 119}{When you do not use the dataset, say "I can't answer this question with the data, but I found this:" You will use pandas and seaborn libraries to write Python code which prints a single PNG image in a bytes64 representation. You will then also print an alt-text caption for the chart.}}
\texttt{\textcolor[RGB]{217, 95, 2}{Let's work responses out step by step to be sure you have the right answer.}}

\texttt{\textcolor[RGB]{102, 102, 102}{The dataset: [DATASET DICTIONARY]}}

\texttt{\textcolor[RGB]{230, 171, 2}{[INPUT-OUTPUT EXAMPLES]}}

Although Data Threads is prompted to output a \textbf{\textcolor[RGB]{217, 95, 2}{chain-of-thought}} answer, this pattern may be superfluous for code synthesis since CoT is inherent to computer programs \cite{}. The previously generated \textbf{\textcolor[RGB]{102, 102, 102}{dataset dictionary}} is included as a markdown table, as well as two \textbf{\textcolor[RGB]{230, 171, 2}{input-output examples}} which correctly output a desired image and caption and are agnostic to data semantics. The example inputs were: ``How many rows are in the dataset?'' and ``Plot the distribution of every continuous measure.'' Appendix A contains the corresponding output examples.

\paragraph{Instructions in a Thread}

\texttt{\textcolor[RGB]{117, 112, 179}{Today we are being asked to revise the following code.}}
\texttt{\textcolor[RGB]{27, 158, 119}{The revised code should print a new chart in a bytes64 PNG representation and print a new alt-text caption in the same way as the original code.}}

\texttt{\textcolor[RGB]{230, 171, 2}{The code: [ORIGINAL CODE]}} 

\texttt{\textcolor[RGB]{102, 102, 102}{The dataset [FILENAME] contains: [DATASET DICTIONARY]}}

In a thread, the user may ask to change visual encodings or make stylistic changes.
They might also ask the model to present additional data columns, to aggregate the data in a new way, or to filter the data, which again requires \textbf{\textcolor[RGB]{102, 102, 102}{information about the dataset}}.
However, the design of this instruction ensures that each user prompt is interpreted to be a question or a command that continues or modifies a specific analysis (\textbf{\textcolor[RGB]{230, 171, 2}{the original code}}), as opposed to starting a new analysis that will require the synthesis of fundamentally different code.

\subsubsection{Synthesizing Code} 
GPT-3.5 responds to the instruction prompt, prior conversation history, and the new analytic prompt with either a text response or visualization code.
The generated code will encompass various aspects of visual data analysis including data retrieval and processing using \texttt{pandas}. 
Data modeling and visualization are handled using the seaborn package and its extensions \texttt{statsmodels}, \texttt{scipy}, and \texttt{fastcluster}.
Even when the model outputs code, the response may contain superfluous text such as ``Sure! I can do that for you.''
Data Threads filters out these responses and instead prints an informative caption that accompanies the generated Python code.

Code might be scattered across a response, especially if the model narrates its chain of thought accompanied by lines of code.
If there are multiple code blocks and only the first one contains import statements, Data Threads conjoins all lines of code into a summative code block.
If more than one code block includes import statements, it returns the last summative code block that includes import statements.
Finally, the code is programmatically cleaned to render a PNG image correctly and checked for proper indentation.

\subsubsection{Executing Code}
The generated and cleaned code will print the output visualization as a Bytes64 string representation of a PNG image such that it can simply be inserted as data to an HTML image tag.
When the code is executed in Python, the server captures images and captions printed to the standard output stream while handling various scenarios such as successes, syntax errors, or execution errors.
Syntax errors implies that the model did not output a code block as a response to the user's prompt, and is therefore rendered as a simple text response.
All other errors signal a system error to the user and cue the, to either Redo or Undo their request.

